The differences of damage initiation and accumulation of DP steels: a numerical and experimental analysis

Many studies have examined the damage behaviour of dual-phase steels already. It is a topic of high interest, since understanding the mechanisms of damage during forming processes enables the production of steels with improved properties and damage tolerance. However, the focus was rarely on the comparison between representatives of this steel class, and the numerical simulation for the quantification of damage states was not thoroughly used. Therefore, this study compares the damage initiation and accumulation of two dual-phase steels (DP800 and DP1000), which are used in the automotive industry. Additionally, parameter sets of a phenomenological damage mechanics model with coupled damage evolution are calibrated for each material. The combined analysis reveals an earlier initiation of damage for the DP800, where the damage accumulation phase is prolonged. For DP1000 the damage nucleates only shortly before material failure. The material model is able to correctly predict the behaviour, while experimental analysis confirms the prediction via light optical and SEM metallography.

==> g.tex <==
newpath
  20 20 moveto
  20 220 lineto
  220 220 lineto
  220 20 lineto
closepath
2 setlinewidth
gsave
  .4 setgray fill
grestore
stroke
grestore

